HCQA @ Ego4D EgoSchema Challenge 2024

In this report, we present our champion solution for Ego4D EgoSchema Challenge in CVPR 2024. To deeply integrate the powerful egocentric captioning model and question reasoning model, we propose a novel Hierarchical Comprehension scheme for egocentric video Question Answering, named HCQA. It consists of three stages: Fine-grained Caption Generation, Context-driven Summarization, and Inference-guided Answering. Given a long-form video, HCQA captures local detailed visual information and global summarised visual information via Fine-grained Caption Generation and Context-driven Summarization, respectively. Then in Inference-guided Answering, HCQA utilizes this hierarchical information to reason and answer given question. On the EgoSchema blind test set, HCQA achieves 75% accuracy in answering over 5,000 human curated multiple-choice questions. Our code will be released at https://github.com/Hyu-Zhang/HCQA.

==> 1_intro.tex <==
\section{Introduction}
\label{sec:intro}

The Ego4D~\cite{grauman2022ego4d} EgoSchema challenge involves choosing the correct answer from five options based on a three-minute-long egocentric video and its related question. The evaluation of this challenge is performed on the EgoSchema dataset~\cite{mangalam2024egoschema}, which consists of over 5,000 human curated multiple-choice question answer pairs, spanning over 250 hours of real video data, covering a very broad range of natural human activity and behavior.
Therefore, this challenge is particularly interesting for evaluating long-context understanding, as it benefits from long ``temporal certificate'' lengths, i.e. the minimum video duration a human needs to answer the question accurately~\cite{balavzevic2024memory,10.1145/3503161.3548020}.

Existing work can be broadly categorized into two groups: 1) train a powerful question answering model for egocentric videos~\cite{papalampidi2023simple, wang2024internvideo2, reid2024gemini,pmlr-v235-zhang24aj}. This approach tends to perform better in capturing details in specific fields. However, this is often limited by large-scale data as well as time and resources. 2) fine-tune a large language model (LLM) via prompt~\cite{zhang2023simple,wang2023lifelongmemory,wang2024videoagent,li2022emocaps,li2024optimus,li2024enhancing,li2023unisa}. This method opens up new solution ideas to leverage existing strong LLM for adapting downstream tasks. Although this approach may be limited by LLM itself to achieve optimal performance, it requires much less computational resources and time, as well as capitalizing on the extensive knowledge embedded in LLM. Therefore, considering the time cost, we adopt the second approach to design our solution.

In Table~\ref{tab:leaderboard}, the baseline LifelongMemory~\cite{wang2023lifelongmemory} achieves the optimal performance in the available methods by applying the effective captioning model LaViLa~\cite{zhao2023learning} and the reasoning model GPT-4\footnote{\url{https://openai.com/index/gpt-4/}.}. However, we find that this method does not establish a temporal correlation between the different captions such that GPT-4 is unable to fully understand the visual scene and complete activity reflected by the captions. At the same time, in-context learning is not introduced, which has been well demonstrated to lead LLM to better perform new tasks.

Therefore, to address the above limitations, we propose a hierarchical comprehension scheme, referred to as HCQA, which incorporates both context-driven summarization and inference-guided answering. Summarization motivates the LLM to better understand the temporal information of the scene, and in-context learning makes it easier for the LLM to understand and perform EgoSchema task. By applying this simple but effective program, we surpass other teams in this challenge and our pipeline achieves a significant improvement compared to the best baseline LifelongMemory (i.e., 68\% $\rightarrow$ 75\% on accuracy in Table~\ref{tab:leaderboard}).



\begin{figure*}[t]
  \centering
  % \fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
   \includegraphics[width=\linewidth]{sec/method_v3.pdf}
   \caption{An illustration of our multi-stage pipeline.}
   \label{fig:method}
\end{figure*}





==> 2_formatting.tex <==
\section{Methodology}
\label{sec:formatting}
As shown in Figure \ref{fig:method}, 
the whole process can be described as follows: 
Given a long-form video, HCQA first transforms it into multiple local clip captions, then adopts these as input to generate a global temporal summary, and finally leverage these hierarchical descriptions to predict the answer to a given question.

% we propose a novel \textbf{H}ierarchical \textbf{C}omprehension scheme
% for egocentric video \textbf{Q}uestion \textbf{A}nswering, named \textbf{HCQA}. It consists of three phases: Fine-Grained Caption Generation, Context-Driven Summarization, and Infer-Guided Answering. 
% Given a long-form video, HCQA first captures the visual information of segmented clips through the Fine-Grained Caption Generation module. Then, it uses the Context-Driven Summarization module to summarize the captions into a global description of the video. Finally, leveraging these hierarchical visual information, the Infer-Guided Answering module infers and provides answers to the questions.

\noindent\textbf{Fine-grained Caption Generation}.
To obtain detailed visual information of the video, we segment a 180-second video into clips at 4-second intervals, resulting in 45 video clips. Then, we employ LaViLa \cite{zhao2023learning} as our captioning model, which is a excellent vision-language model pretrained on Ego4D \cite{grauman2022ego4d}. Specifically, we uniformly sample 4 frames from each clip and use LaViLa to produce five corresponding textual captions for diversity. In this way, we can obtain 45$\times$5 captions, which could provide sufficient visual semantics for the subsequent question answering.

\noindent\textbf{Context-driven Summarization}.
The original caption provides a detailed description of each clip in the video, however these descriptions are discrete and unrelated. In order to integrate these captions from the temporal dimension, we propose in-context aware caption summarization~\cite{10239469}, which couples these captions to establish associations and aggregates them into an overall overview of the video. Specifically, we employ prompt learning to instruct GPT-4o\footnote{\url{https://openai.com/index/hello-gpt-4o/}.} to generate a comprehensive overview of a video based on given captions. To achieve a more accurate and detailed video summary, we employ in-context learning \cite{brown2020language,dai2022can} in our approach. Empirically, we set the number of cases for in-context learning to 1. By leveraging this high-quality case as references, we guide the model to consider both local and global information during the summary generation process.

\noindent\textbf{Inference-guided Answering}.
To enhance the model's reasoning ability, we propose using the Chain-of-Thought (CoT) method \cite{wei2022chain}. This method guides the model to capture key information from captions and summaries, explicitly outputting the reasoning process for questions~\cite{10.1145/3474085.3475234,zhang2023uncovering}. Consequently, it improves the model's accuracy in answering complex visual questions. 
Notably we also employ in-context learning, using three high-quality examples from the EgoSchema subset.
Moreover, inspired by the impact of reflection mechanism \cite{shinn2023reflexion} on enhancing the performance of LLM, we incorporate a reflection mechanism into the question answering process. Specifically, after generating an answer, we prompt the model to output a confidence score for its response. If the confidence is below a certain threshold (5 in our settings), we require the model to reflect on its previous answer, assess any potential errors, and correct it if necessary. 
% For Infer-Guided Answering, we utilize GPT-4o with a temperature setting of 0.1.

%In summary, after obtaining fine-grained captions and a global summary, we prompt GPT-4o to complete reasoning, answering, and confidence evaluation step-by-step, using Chain-of-Thought \cite{wei2022chain} approach.




==> 3_finalcopy.tex <==
\section{Experiment}

\subsection{Performance Comparison}
Table~\ref{tab:leaderboard} displays the existing methods as well as our primary leaderboard results. From the results, we can see that the optimal existing method LifelongMemory achieves 68\% accuracy on the EgoSchema full set, and yet this approach can only be ranked 5th on the public leaderboard. 
Our framework achieves a accuracy of 75\%, ranked first, significantly outperforming all the other teams and existing work. This thereby proves the superiority of our method.

\subsection{Solution Evolution}
% In this section, we present the iterative process of our scheme in Table~\ref{tab:ablation} and also show a comparison of different captioning models and reasoning models in Table~\ref{tab:captioner} and~\ref{tab:llm}.

Table~\ref{tab:ablation} presents the iterative process of our solution. We first utilize the LifelongMemory~\cite{wang2023lifelongmemory} as our backbone and test its results on the EgoSchema dataset. To enhance the expression of video clip, we increase the number of caption from 1 to 3, achieving an absolute improvement of 2.4\%. After observing this obvious leap, we further increase the number of caption while introducing an example for in-context learning. And in order to strengthen the understanding of the LLM for global temporal information, we add inductive summarization in addition to predicting answers. This produces a gain of 3.2\%. In order to reduce the difficulty of performing simultaneous summarization and prediction for LLM, we separate the process into two phases: summarization followed by prediction. Although the length of the generated summaries increased significantly, this does not result in a significant accuracy improvement. Considering that one example may not provide guidance for different samples, we enrich the original example by filtering three typical examples from the subset, which gains 0.5\% increments. It is worth noting that all of the above solutions generate reason and confidence in addition to predicting answer. For uncertain predictions, i.e., low confidence, we ask LLM to reflect on and re-predict previous answers. This results in a 0.2\% benefit.

\begin{table}
  \caption{Performance comparison of existing work and the top five teams on the public leaderboard.}
  \centering
  \begin{tabular}{ccc}
    \toprule
    Method & Rank & Accuracy \\
    \midrule
    % FrozenBiLM~\cite{yang2022zero} & - & 0.27\\
    mPLUG-Owl~\cite{ye2023mplug} & -&0.31\\
    LongViViT~\cite{papalampidi2023simple}& -&0.33\\
    InternVideo2~\cite{wang2024internvideo2} &-& 0.41\\
    LLoVi~\cite{zhang2023simple} &-& 0.50\\
    VideoAgent~\cite{wang2024videoagent} & -&0.54\\
    ProViQ~\cite{choudhury2023zero}&-&0.57\\
    Gemini 1.5 Pro~\cite{reid2024gemini} & -&0.63\\
    LifelongMemory~\cite{wang2023lifelongmemory}&-&0.68\\
    \midrule
    Host\_82934\_Team & 5 & 0.64\\
    VeryLongVQA & 4 & 0.69\\
    PaMsEgoAI & 3& 0.71\\
    GMMV & 2 & 0.74\\
    \midrule
   HCQA (iLearn) & 1& \textbf{0.75}\\
    \bottomrule
  \end{tabular}
  \label{tab:leaderboard}
\end{table}

\subsection{Ablation Study}
In Table~\ref{tab:captioner}, we investigate the effects of different captioning and reasoning models. The results show that LaViLa achieves the best results over EgoVLP~\cite{lin2022egocentric} and VideoRecap~\cite{islam2024video} under consistent application of GPT-3.5. After fixing LaViLa for the captioning model, we also study the effectiveness of different reasoning models. These results suggest that GPT-4o's reasoning is superior to that of GPT-3.5 and GPT-4, leading to a superior performance.

\subsection{Case Analysis}
Figure~\ref{fig:case} shows two examples of our framework, including a successful one and a failed one. In Figure~\ref{fig:success_case}, captions and summary are correctly generated to describe the camera wearer's short-term actions and long-term activities, i.e., cleaning dishes and others. With the hierarchical narrations, our framework understands the complete activity and correctly answers the question with appropriate explanations. In Figure~\ref{fig:failure_case}, although the video content is appropriately described, our reasoning model does not predict the correct answer. This may be due to the fact that the words ``card game" and ``board game" in the answer are too close to each other, causing the LLM to fail to specify the boundary between the two.


% \begin{table}
%   \centering
%   \begin{tabular}{ccc}
%     \toprule
%     Method & Subset & Full \\
%     \midrule
%     \textit{Zero-shot}\\
%     FrozenBiLM~\cite{yang2022zero} & - & 0.27\\
%     mPLUG-Owl~\cite{ye2023mplug} & -&0.31\\
%     InternVideo~\cite{wang2022internvideo} &-&0.32\\
%     LongViViT~\cite{papalampidi2023simple}& 0.57&0.33\\
%     TimeSformer~\cite{bertasius2021space} & -&0.38\\
%     TimeMamba~\cite{chen2024video} & -&0.39\\
%     InternVideo2~\cite{wang2024internvideo2} &-& 0.41\\
%     Vamos~\cite{wang2023vamos} &-& 0.48\\
%     LLoVi~\cite{zhang2023simple} &0.58& 0.50\\
%     MoReVQA~\cite{min2024morevqa}&-&0.52\\
%     VideoAgent~\cite{wang2024videoagent} & 0.60&0.54\\
%     Gemini 1.0 Pro~\cite{reid2024gemini}&-& 0.56\\
%     MovieChat+~\cite{song2024moviechat+}&-&0.56\\
%     ProViQ~\cite{choudhury2023zero}&-&0.57\\
%     Gemini 1.0 Ultra~\cite{reid2024gemini} &-& 0.62\\
%     Gemini 1.5 Pro~\cite{reid2024gemini} & -&0.63\\
% LifelongMemory~\cite{wang2023lifelongmemory}&-&0.68\\
%     \midrule
%     \textit{Few-shot}\\
%     MC-ViT-L~\cite{balavzevic2024memory}&0.63 &0.44\\
%     LLoVi~\cite{zhang2023simple} &-& 0.53\\
%     \bottomrule
%   \end{tabular}
%   \caption{Results.  Ours is better.}
%   \label{tab:existing_work}
% \end{table}




\begin{table*}
  \caption{Performance comparison on EgoSchema full set between our different solutions.}
  \centering
  \begin{tabular}{cccc}
    \toprule
    Order & Accuracy & Caption Number & Modification \\
    \midrule
    1 & 0.684 &1& Follow LifelongMemory~\cite{wang2023lifelongmemory} pipeline\\
    2 & 0.708 (0.024$\uparrow$) &3& Replace one caption with three per clip\\
    3 & 0.740 (0.032$\uparrow$) &5& Adopt one-shot in-context learning and reason both summary and answer\\
    4 & 0.741 (0.001$\uparrow$) &5&Reason the summary first and then predict the answer\\
    5 & 0.746 (0.005$\uparrow$) &5&Adopt three-shot in-context learning\\
    6 & 0.748 (0.002$\uparrow$) &5&Perform reflection for low-confidence sample\\
    \bottomrule
  \end{tabular}
  \label{tab:ablation}
  \vspace{-1ex}
\end{table*}

\begin{figure}
  \centering
  \begin{subfigure}{\linewidth}
    \includegraphics[width=\linewidth]{sec/case1.pdf}
    \caption{Success case.}
    \label{fig:success_case}
  \end{subfigure}
  \hfill
  \begin{subfigure}{\linewidth}
    \includegraphics[width=\linewidth]{sec/case2.pdf}
    \caption{Failure case.}
    \label{fig:failure_case}
  \end{subfigure}
  \caption{Two examples of our framework on EgoSchema subset.}
  \label{fig:case}
  \vspace{-1em}
\end{figure}

% \begin{figure}[t]
%   \centering
%   \fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
%    %\includegraphics[width=0.8\linewidth]{egfigure.eps}

%    \caption{Example of caption.
%    It is set in Roman so that mathematics (always set in Roman: $B \sin A = A \sin B$) may be included without an ugly clash.}
%    \label{fig:onecol}
% \end{figure}

\begin{table}
  \caption{Accuracy of our framework on EgoSchema subset with different captioning and reasoning model.}
  \centering
  \begin{tabular}{ccccc}
    \toprule
    Captioning Model & Reasoning Model & Accuracy \\
    \midrule
    EgoVLP~\cite{lin2022egocentric}& GPT-3.5 & 0.466\\
    % BLIP-2 & -& 0.467\\
    LaViLa~\cite{zhao2023learning} & GPT-3.5&\textbf{0.518}\\
    VideoRecap~\cite{islam2024video} & GPT-3.5&0.512\\
    \midrule
    LaViLa~\cite{zhao2023learning} & GPT-4 & 0.583\\
    LaViLa~\cite{zhao2023learning} & GPT-4o & \textbf{0.588}\\
    \bottomrule
  \end{tabular}
  \label{tab:captioner}
  \vspace{-1ex}
\end{table}

% \begin{table}
%   \centering
%   \begin{tabular}{ccccc}
%     \toprule
%     Reasoning Model & Model Size & Accuracy \\
%     \midrule
%     Llama2-70B & 70B & 0.506\\
%     GPT-3.5 & 175B & 0.518\\
%     GPT-4 & - & 0.583 \\
%     GPT-4o & - & \textbf{0.588} \\
%     \bottomrule
%   \end{tabular}
%   \caption{Accuracy of our framework on subset with different reasoning model. All baselines use the same captioning model, i.e., LaViLa.}
%   \label{tab:llm}
% \end{table}
